A Cyclic Proof System for HFLN

A cyclic proof system allows us to perform inductive reasoning without explicit inductions. We propose a cyclic proof system for HFLN, which is a higher-order predicate logic with natural numbers and alternating fixed-points. Ours is the first cyclic proof system for a higher-order logic, to our knowledge. Due to the presence of higher-order predicates and alternating fixed-points, our cyclic proof system requires a more delicate global condition on cyclic proofs than the original system of Brotherston and Simpson. We prove the decidability of checking the global condition and soundness of this system, and also prove a restricted form of standard completeness for an infinitary variant of our cyclic proof system. A potential application of our cyclic proof system is semi-automated verification of higher-order programs, based on Kobayashi et al.'s recent work on reductions from program verification to HFLN validity checking.

==> completeness.tex <==
\setcounter{section}{4}
\section{Proof of \autoref{completeness}} \label{ap: completeness}
\begin{definition}[Schedule]
  \emph{A schedule element} is a formula of the form $\varphi \lor \psi, \varphi \land \psi, (\lambda x. \varphi) \, \psi \, \vec{\psi}, (\sigma x. \varphi) \, \vec{\psi}$.
  We call $(E_i)_{i \geq 0}$ \emph{a schedule} if $E_i$ is a schedule element for all $i$ and every schedule element appears infinitely often in $(E_i)_{i \geq 0}$.
\end{definition}
There exists a schedule and we fix the one.

\begin{definition}[$T_\omega$] \label{def: tomega}
  Let $\Gamma \vdash \Delta$ be a valid sequent which does not have higher-order free variables.
  Then we will define trees $(T_i)_{i \geq 0}$ whose root is $\Gamma \vdash \Delta$ inductively by using a schedule $(E_i)_{i \geq 0}$.
  First, $T_0$ is defined as below:
  \begin{center}
    $T_0 :=$
    \AxiomC{$N \, x_0,..., N \, x_n, \Gamma \vdash \Delta$}
    \RightLabel{(Nat)}
    \UnaryInfC{$\Gamma \vdash \Delta$}
    \DisplayProof
  \end{center}
  where $x_0, ..., x_n$ are all free natural number variables in $\Gamma \cup \Delta$.

  Assume $T_i$ is already defined.
  Then we define $T_{i+1}$ in $T_i$ by repracing each open leaf $\Gamma' \vdash \Delta'$ to the following tree:
  Let $\sim$ be the equivalence relation generated by $\{ (s, t) \mid s = t \in \Gamma' \}$:
  \begin{itemize}
    \item If there exists a formula $\varphi \in \Gamma' \cap \Delta'$:

      \begin{center}
        \AxiomC{}
        \RightLabel{(Axiom)}
        \UnaryInfC{$\varphi \vdash \varphi$}
        \RightLabel{(WK)}
        \UnaryInfC{$\Gamma' \vdash \Delta'$}
        \DisplayProof
      \end{center}

    \item If $(s=t) \in \Gamma'$, $s \sim \mathbf{S}^n\mathbf{Z}$ and $t \sim \mathbf{S}^m\mathbf{Z}$ for some different natural numbers $n < m$:

      \begin{center}
        \AxiomC{}
        \RightLabel{(P1)}
        \UnaryInfC{$\mathbf{Z} = \mathbf{S}^{(m-n)}\mathbf{Z} \vdash$}
        \RightLabel{(P2)}
        \UnaryInfC{$\mathbf{S}^n\mathbf{Z} = \mathbf{S}^m\mathbf{Z} \vdash$}
        \RightLabel{($=$L, Wk)}
        \UnaryInfC{$\Gamma' \vdash \Delta'$}
        \DisplayProof
      \end{center}

    \item If $(s=t) \in \Delta'$ and $s \sim t$:

      \begin{center}
        \AxiomC{}
        \RightLabel{($=$R)}
        \UnaryInfC{$ \vdash s = s$}
        \RightLabel{($=$L, Wk)}
        \UnaryInfC{$\Gamma' \vdash \Delta'$}
        \DisplayProof
      \end{center}

    \item If $f \, \vec{s} \in \Gamma', f \, \vec{t} \in \Delta'$ and $\vec{s} \sim \vec{t}$:

      \begin{center}
        \AxiomC{}
        \RightLabel{($=$R)}
        \UnaryInfC{$f \, \vec{s} \vdash f \, \vec{s}$}
        \RightLabel{($=$L, Wk)}
        \UnaryInfC{$\Gamma' \vdash \Delta'$}
        \DisplayProof
      \end{center}

    \item Otherwise:
      This replacement is preformed in such a way that each formula is targeted fairly.
      Therefore, each formula is expanded at some point.
      \begin{itemize}
      \item Case ($E_i \equiv \varphi \lor \psi$):
        \begin{itemize}
          \item if $E_i \in \Gamma'$:
            \begin{center}
            \AxiomC{$\Gamma', \varphi \vdash \Delta'$}
            \AxiomC{$\Gamma', \psi \vdash \Delta'$}
            \RightLabel{($\lor$L)}
            \BinaryInfC{$\Gamma', \varphi \lor \psi \vdash \Delta'$}
            \RightLabel{(Ctr)}
            \UnaryInfC{$\Gamma' \vdash \Delta'$}
            \DisplayProof
            \end{center}

          \item if $E_i \in \Delta'$:
            \begin{center}
              \AxiomC{$\Gamma'\vdash \varphi, \psi, \Delta'$}
              \RightLabel{($\lor$R)}
              \UnaryInfC{$\Gamma' \vdash \varphi \lor \psi, \Delta'$}
              \RightLabel{(Ctr)}
              \UnaryInfC{$\Gamma' \vdash \Delta'$}
              \DisplayProof
            \end{center}
        \end{itemize}
      \item Case $(E_i \equiv \varphi \land \psi)$:
        The tree is defined in the similar way to the case $E_i \equiv \varphi \lor \psi$.

      \item Case $(E_i \equiv (\lambda x. \varphi) \, \psi \, \vec{\psi})$:
        \begin{itemize}
          \item if $E_i \in \Gamma'$:
            \begin{center}
              \AxiomC{$\Gamma', \varphi[\psi/x] \, \vec{\psi} \vdash \Delta'$}
              \RightLabel{($\lambda$L)}
              \UnaryInfC{$\Gamma', (\lambda x. \varphi) \, \psi \, \vec{\psi} \vdash \Delta'$}
              \RightLabel{(Ctr)}
              \UnaryInfC{$\Gamma' \vdash \Delta'$}
              \DisplayProof
            \end{center}

          \item if $E_i \in \Delta'$:
            \begin{center}
              \AxiomC{$\Gamma' \vdash \varphi[\psi/x] \, \vec{\psi}, \Delta'$}
              \RightLabel{($\lambda$R)}
              \UnaryInfC{$\Gamma' \vdash (\lambda x. \varphi) \, \psi \, \vec{\psi}, \Delta'$}
              \RightLabel{(Ctr)}
              \UnaryInfC{$\Gamma' \vdash \Delta'$}
              \DisplayProof
            \end{center}
        \end{itemize}
      \item Case $(E_i \equiv (\sigma x. \varphi) \, \vec{\psi})$:
        \begin{itemize}
          \item if $E_i \in \Gamma'$:
            \begin{center}
              \AxiomC{$\Gamma', \varphi[\sigma x. \varphi/x] \, \vec{\psi} \vdash \Delta'$}
              \RightLabel{($\sigma$L)}
              \UnaryInfC{$\Gamma', (\sigma x. \varphi) \, \vec{\psi} \vdash \Delta'$}
              \RightLabel{(Ctr)}
              \UnaryInfC{$\Gamma' \vdash \Delta'$}
              \DisplayProof
            \end{center}

          \item if $E_i \in \Delta'$:
            \begin{center}
              \AxiomC{$\Gamma' \vdash \varphi[\sigma x. \varphi/x] \, \vec{\psi}, \Delta'$}
              \RightLabel{($\sigma$R)}
              \UnaryInfC{$\Gamma' \vdash (\sigma x. \varphi) \, \vec{\psi}, \Delta'$}
              \RightLabel{(Ctr)}
              \UnaryInfC{$\Gamma' \vdash \Delta'$}
              \DisplayProof
            \end{center}
        \end{itemize}
    \end{itemize}
  \end{itemize}
  Note that for all $i \geq 0$,
  $T_i \subseteq T_{i+1}$
  and each sequent of an open leaf in $T_{i+1}$ includes the sequent of the corresponding leaf in $T_i$.
  We define $T_\omega$ to be $\lim_{i \to \infty} T_i$.
\end{definition}

For all $i \geq 0$, all open leaves in $T_i$ includes $N \, x_0, ..., N \, x_n, \Gamma \vdash \Delta$
thus they are finally replaced by some schedule element $E_j$.
Hence $T_\omega$ does not have open leaves and $T_\omega$ is a pre-proof.

We aim to prove the pre-proof $T_\omega$ satisfies the global trace condition.
\begin{definition}[$\Gamma_\omega \vdash \Delta_\omega, \rho_\omega$] \label{def: rhoomega}
  Assume $T_\omega$ in \autoref{def: tomega} is not a proof.
  $T_\omega$ is a pre-proof thus there is an infinite path $\pi = (\pi_i)_{i \geq 0}$ in $T_\omega$ which does not satisfy the global trace condition.

  We define $\Gamma_\omega \vdash \Delta_\omega$ as $\lim_{i \to \infty} (\Gamma_i \vdash \Delta_i)$ where $\Gamma_i \vdash \Delta_i$ is the sequent of $\pi_i$.

  A valuation $\rho_\omega$ of $\Gamma_\omega \vdash \Delta_\omega$ is defined as below:
  \begin{align*}
    \rho_\omega(x^\mathbf{N}) &:= n \text{ where }(x = \mathbf{S}^n\mathbf{Z}) \in \Gamma_\omega \\
    \rho_\omega(x^\mathbf{\Omega}) &:= \begin{cases} \top & \text{if } x \in \Gamma_\omega \\ \bot & \text{otherwise}\end{cases} \\
    \rho_\omega(f^{\mathbf{N}^n \to \mathbf{\Omega}}) &:= \{ \llbracket \vec{x} \rrbracket_{\rho_\omega} \mid f \, \vec{x} \in \Gamma_\omega \}
  \end{align*}
  All free natural number variables in $\Gamma_\omega \cup \Delta_\omega$ are free variables in $\Gamma \cup \Delta$.
  For all free natural number variables $x \in \Gamma \cup \Delta$,
  there exists $n \in \mathbb{N}$ such that $(x = \mathbf{S}^n\mathbf{Z}) \in \Gamma_\omega$.
  If there is no such $n \in \mathbb{N}$, $N \, x$ is unfolded infinitely often in $\pi$ and we can trace the left $\mu$ in $N$.
  This contradicts that $\pi$ does not satisfy the global trace condition.
  Besides, such $n \in \mathbb{N}$ is unique because if $x = \mathbf{S}^n\mathbf{Z}, x = \mathbf{S}^m\mathbf{Z} \in \Gamma_\omega$ and $n, m$ are different numbers then $\pi$ is not infinite by the way of the construction of $T_\omega$.
  Therefore, the valuation $\rho_\omega(x^\mathbf{N})$ is well-defined.
\end{definition}

\begin{lemma} \label{lem: rhoomega}
  If $\varphi \in \Gamma_\omega$ then $\llbracket \varphi \rrbracket_{\rho_\omega} = \top$ and
  if $\varphi \in \Delta_\omega$ then $\llbracket \varphi \rrbracket_{\rho_\omega} = \bot$.
\end{lemma}
\begin{proof}
  We give the proof only for the first claim.

  Assume there exists a formula $\varphi \in \Gamma_\omega$ such that $\llbracket \varphi \rrbracket_{\rho_\omega} = \bot$.
  Let $j$ be a number such that $\varphi \in \pi_j$.
  We will show that there exists a left $\mu$-trace $(\tau_i)_{i \geq j}$ in $\pi$ starting from $\varphi$.

  We define $(\tau_i)_{i \geq j}$ and $(\tau_i')_{i \geq j}$ which satisfy the following conditions:
  \begin{enumerate}
    \item $\tau_i \in \Gamma_i$;
    \item we can get $\tau_i$ by forgetting ordinal numbers of $\tau_i'$;
    \item each $\nu$ in $\tau_i'$ has an ordinal number;
    \item $\llbracket \tau_i' \rrbracket_{\rho_\omega} = \bot$ where $\llbracket . \rrbracket$ for $\nu^\alpha$ is the same as \autoref{ap: soundness};
    \item each ordinal number in $\tau_{i+1}'$ is less than or equal to the corresponding ordinal number in $\tau_i'$.
  \end{enumerate}

  The definition of $(\tau_i)_{i \geq j}$ and $(\tau_i')_{i \geq j}$ as below:
  \begin{itemize}
    \item $\tau_j := \varphi$.
      Because $\llbracket \varphi \rrbracket_{\rho_\omega} = \bot$, we can get $\varphi'$ which satisfies $\llbracket \varphi' \rrbracket_{\rho_\omega} = \bot$ by assigning ordinal numbers to all $\sigma$ in $\varphi$.
    \item Assume $\tau_i$ and $\tau_i'$ are defined.
      Below, $\psi'$ means the corresponding annotated formula.
      \begin{itemize}
        \item If $\tau_i \equiv x$:

          Since $x \in \Gamma_i$, $\llbracket x \rrbracket_{\rho_\omega} = \top$ because of the definition of $\rho_\omega$.
          By the assumption of $\tau_i'$,
          $\llbracket (x)' \rrbracket_{\rho_\omega} = \llbracket x \rrbracket_{\rho_\omega} = \bot$.
          This is a contradiction.

        \item If $\tau_i \equiv (s=t)$:

          By the assumption of $\tau_i'$,
          $\llbracket (s=t)' \rrbracket_{\rho_\omega} = \llbracket s=t \rrbracket_{\rho_\omega} = \bot$.
          Then $\pi$ is not infinite because of the construction of $T_\omega$.
          This contradicts the fact that $\pi$ is an infinite path.

        \item If $\tau_i \equiv f \, \vec{t}$:

          Since $f \, \vec{t} \in \Gamma_i$, $\llbracket f \, \vec{t} \rrbracket_{\rho_\omega} = \top$ because of the definition of $\rho_\omega$.
          By the assumption of $\tau_i'$,
          $\llbracket (f \, \vec{t})' \rrbracket_{\rho_\omega} = \llbracket f \, \vec{t} \rrbracket_{\rho_\omega} = \bot$.
          This is a contradiction.

        \item If $E_i \not \equiv \tau_i$ then $\tau_{i+1} := \tau_i$ and $\tau_{i+1}' := \tau_i'$.
        \item Otherwise:
          \begin{itemize}
        \item Case $\tau_i \equiv (\psi \lor \chi)$:

          Since $\llbracket \psi' \lor \chi' \rrbracket_{\rho_\omega} = \bot$,
          $\llbracket \psi' \rrbracket_{\rho_\omega} = \llbracket \chi' \rrbracket_{\rho_\omega} = \bot$.
          $\tau_{i+1} := \psi, \tau_{i+1}' := \psi'$ if $\pi$ goes to the left leaf,
          and otherwise $\tau_{i+1} := \chi, \tau_{i+1}' := \chi'$.
          In each case, $\llbracket \tau_{i+1}' \rrbracket_{\rho_\omega} = \bot$ holds.

        \item Case $\tau_i \equiv (\psi \land \chi)$:

          Since $\llbracket \psi' \land \chi' \rrbracket_{\rho_\omega} = \bot$, either $\llbracket \psi' \rrbracket_{\rho_\omega}$ or $\llbracket \chi' \rrbracket_{\rho_\omega}$ is $\bot$.

          $\tau_{i+1} := \psi, \tau_{i+1}' := \psi'$ if $\llbracket \psi' \rrbracket_{\rho_\omega} = \bot$, and otherwise $\tau_{i+1} := \chi, \tau_{i+1}' := \chi'$.

        \item Case $\tau_i \equiv (\lambda x. \psi) \, \chi \, \vec{\theta}$:

          $\tau_{i+1} := \psi[\chi/x] \, \vec{\theta}, \tau_{i+1}' := \psi'[\chi'/x] \, \vec{\theta'}$

          then $\llbracket \psi'[\chi'/x] \, \vec{\theta'} \rrbracket_{\rho_\omega} = \llbracket (\lambda x. \psi') \, \chi' \, \vec{\theta'} \rrbracket_{\rho_\omega} = \bot$.

        \item Case $\tau_i \equiv (\mu x. \psi) \, \vec{\theta}$:

          $\tau_{i+1} := \psi[\mu x. \psi/x] \, \vec{\theta}$, $\tau_{i+1}' := \psi'[\mu x. \psi'/x] \, \vec{\theta'}$

          then $\llbracket (\psi'[\mu x. \psi'/x]) \, \vec{\theta'} \rrbracket_{\rho_\omega} = \llbracket (\mu x. \psi') \, \vec{\theta'} \rrbracket_{\rho_\omega} = \bot$.

        \item Case $\tau_i \equiv (\nu x. \psi) \, \vec{\theta}$:

          Let $\alpha$ be the ordinal number which assigned to the head $\nu$ of $(\nu x. \varphi) \, \vec{\psi}$.
          If $\alpha = 0$ then
          $\llbracket (\nu^0 x^T. \varphi') \, \vec{\psi'} \rrbracket_{\rho_\omega}
          = \llbracket (\top_T) \, \vec{\psi'} \rrbracket_{\rho_\omega} = \top$
          and this contradicts the assumption.
          \begin{align*}
          \llbracket (\nu^\alpha x. \psi') \, \vec{\theta'} \rrbracket_{\rho_\omega}
          &= ((\lambda  v. \llbracket \psi' \rrbracket_{\rho_\omega[x \mapsto v]})^{\alpha} \, (\top_n)) \, \llbracket \vec{\theta'} \rrbracket_{\rho_\omega} \\
          &= (\bigwedge_{\beta < \alpha} (\lambda v. \llbracket \psi' \rrbracket_{\rho_\omega[x \mapsto v]}) \, ((\lambda v. \llbracket \psi' \rrbracket_{\rho_\omega[x \mapsto v]})^{\beta} \, (\top_n))) \, \llbracket \vec{\theta'} \rrbracket_{\rho_\omega} \\
          &= \bot
          \end{align*}

          There exists $\beta < \alpha$ such that
          $((\lambda v. \llbracket \psi' \rrbracket_{\rho_\omega[x \mapsto v]}) \, ((\lambda v. \llbracket \psi' \rrbracket_{\rho_\omega[x \mapsto v]})^{\beta} \, (\top_n))) \, \llbracket \vec{\theta'} \rrbracket_{\rho_\omega} = \bot$.
          $\tau_{i+1} := \psi[\nu x. \psi/x] \, \vec{\theta}$, $\tau_{i+1}' := \psi'[\nu^\beta x. \psi'/x] \, \vec{\theta'}$ then
          \begin{align*}
          \llbracket (\psi'[\nu^\beta x. \psi'/x]) \, \vec{\theta'} \rrbracket_{\rho_\omega}
          &= ((\lambda  v. \llbracket \psi' \rrbracket_{\rho_\omega[x \mapsto v]}) \, (\llbracket \nu^\beta x. \psi' \rrbracket_{\rho_\omega})) \, \llbracket \vec{\theta'} \rrbracket_{\rho_\omega} \\
          &= ((\lambda  v. \llbracket \psi' \rrbracket_{\rho_\omega[x \mapsto v]}) \, ((\lambda v. \llbracket \psi' \rrbracket_{\rho_\omega[x \mapsto v]})^{\beta} \, (\top_n))) \, \llbracket \vec{\theta'} \rrbracket_{\rho_\omega} \\
          &= \bot
          \end{align*}
        \end{itemize}
      \end{itemize}
  \end{itemize}
  If this $(\tau_i)_{i \geq j}$ is a $\nu$-trace,
  there is an infinite sequence $p$ of the trace by the definition of $\nu$-trace.
  For all $n \geq 1$, there is a $\nu_{p[0:n]}$ in some $\tau_i$ and we denote by $\alpha_n$ the ordinal number assigned to this $\nu$.
  By the definition of $(\alpha_n)_{n \geq 1}$ and $(\tau_i)_{i \geq j}$, every odrinal number assigned to $\nu_{p[0:n]}$ is $\alpha_n$,
  for all $n$, there exists $i$ such that $(\tau_i \equiv (\nu_{p[0:n]} x. \psi) \, \vec{\theta}) \to (\tau_{i+1} \equiv (\psi[\nu_{p[0:n+1]} x. \psi/x]) \, \vec{\theta})$.
  Hence $\alpha_n > \alpha_{n+1}$ holds for all $n \geq 1$ so $(\alpha_n)_{n \geq 1}$ is a decreasing sequence of ordinal numbers.
  However, such a sequence does not exist so this is a contradiction.

  By \autoref{lem: uniqueness}, it follows that $(\tau_i)_{i \geq j}$ is a left $\mu$-trace of $\pi$.
  Then this contradicts to the assumption of $\pi$.
\end{proof}

\begin{proof}[Proof (\autoref{completeness}).]
  First, we construct $T_\omega$ from $\Gamma \vdash \Delta$ as \autoref{def: tomega}.
  Assume $T_\omega$ is not a proof
  and we define $\rho_\omega$ as \autoref{def: rhoomega}.
  then \autoref{lem: rhoomega} concludes $\Gamma \not \models_{\rho_\omega} \Delta$ because $\Gamma \subseteq \Gamma_\omega$ and $\Delta \subseteq \Delta_\omega$.
  This contradicts $\Gamma \models \Delta$.
  Thus $T_\omega$ is a proof of $\Gamma \vdash \Delta$.
  Besides, $T_\omega$ is cut-free because of the way of the construction.
\end{proof}

